Mutation of type $D$ friezes

In this article we study mutation of friezes of type $D$. We provide a combinatorial formula for the entries in a frieze after mutation. The two main ingredients in the proof include a certain transformation of a type $D$ frieze into a sub pattern of a frieze of type $A$ and the mutation formula for type $A$ friezes recently found by Baur et al.

==> firezes-5.tex <==
@article{CCS06,
  title={Quivers with relations arising from clusters ({$A_n$} case)},
  author={Caldero, Philippe and Chapoton, Fr\'ed\'eric and Schiffler, Ralf},
  journal={Transactions of the American Mathematical Society},
  volume={358},
  number={3},
  pages={1347--1364},
  year={2006}
}

@incollection{Sch18,
  title={Cluster Algebras from Surfaces},
  author={Schiffler, Ralf},
  booktitle={Homological Methods, Representation Theory, and Cluster Algebras},
  pages={65--99},
  year={2018},
  publisher={Springer}
}

@article{M-G,
    AUTHOR = {Morier-Genoud, Sophie},
     TITLE = {Coxeter's frieze patterns at the crossroads of algebra,
              geometry and combinatorics},
   JOURNAL = {Bull. Lond. Math. Soc.},
  FJOURNAL = {Bulletin of the London Mathematical Society},
    VOLUME = {47},
      YEAR = {2015},
    NUMBER = {6},
     PAGES = {895--938},
      ISSN = {0024-6093},
   MRCLASS = {05E10 (13F60 14M15 16G20 39A70)},
  MRNUMBER = {3431573},
MRREVIEWER = {Kyungyong Lee},
       DOI = {10.1112/blms/bdv070},
       URL = {https://doi.org/10.1112/blms/bdv070},
}


@article {AP,
  title={The cluster category of a surface with punctures via group actions},
  author={Amiot, Claire and Plamondon, Pierre-Guy},
  journal={arXiv preprint arXiv:1707.01834},
  year={2017}
}


@article {BM,
    AUTHOR = {Baur, Karin and Marsh, Robert J.},
     TITLE = {Frieze patterns for punctured discs},
   JOURNAL = {J. Algebraic Combin.},
  FJOURNAL = {Journal of Algebraic Combinatorics. An International Journal},
    VOLUME = {30},
      YEAR = {2009},
    NUMBER = {3},
     PAGES = {349--379},
      ISSN = {0925-9899},
   MRCLASS = {05E15 (13F60)},
  MRNUMBER = {2545501},
       DOI = {10.1007/s10801-008-0161-0},
       URL = {https://doi.org/10.1007/s10801-008-0161-0},
}
		

@article {S,
    AUTHOR = {Schiffler, Ralf},
     TITLE = {A geometric model for cluster categories of type {$D_n$}},
   JOURNAL = {J. Algebraic Combin.},
  FJOURNAL = {Journal of Algebraic Combinatorics. An International Journal},
    VOLUME = {27},
      YEAR = {2008},
    NUMBER = {1},
     PAGES = {1--21},
      ISSN = {0925-9899},
   MRCLASS = {16G10 (05A15 16D90 18E30)},
  MRNUMBER = {2366159},
MRREVIEWER = {Xiuping Su},
       DOI = {10.1007/s10801-007-0071-6},
       URL = {https://doi.org/10.1007/s10801-007-0071-6},
}
		

@book {SchifflerBook,
    AUTHOR = {Schiffler, Ralf},
     TITLE = {Quiver representations},
    SERIES = {CMS Books in Mathematics/Ouvrages de Math\'ematiques de la
              SMC},
 PUBLISHER = {Springer, Cham},
      YEAR = {2014},
     PAGES = {xii+230},
      ISBN = {978-3-319-09203-4; 978-3-319-09204-1},
   MRCLASS = {16G20 (16G70)},
  MRNUMBER = {3308668},
MRREVIEWER = {Alex Martsinkovsky},
       DOI = {10.1007/978-3-319-09204-1},
       URL = {http://dx.doi.org/10.1007/978-3-319-09204-1},
}


@article{baur2018mutation,
  title={Mutation of friezes},
  author={Baur, Karin and Faber, Eleonore and Gratz, Sira and Serhiyenko, Khrystyna and Todorov, Gordana},
  journal={Bulletin des Sciences Mathematiques},
  volume={142},
  pages={1--48},
  year={2018},
  publisher={Elsevier}
}


@article {CC2,
    AUTHOR = {Conway, J. H. and Coxeter, H. S. M.},
     TITLE = {Triangulated polygons and frieze patterns},
   JOURNAL = {Math. Gaz.},
  FJOURNAL = {The Mathematical Gazette},
    VOLUME = {57},
      YEAR = {1973},
    NUMBER = {401},
     PAGES = {175--183},
      ISSN = {0025-5572},
   MRCLASS = {50B30},
  MRNUMBER = {0461270},
       DOI = {10.2307/3615561},
       URL = {https://doi.org/10.2307/3615561},
}

@article {CC1,
    AUTHOR = {Conway, J. H. and Coxeter, H. S. M.},
     TITLE = {Triangulated polygons and frieze patterns},
   JOURNAL = {Math. Gaz.},
  FJOURNAL = {The Mathematical Gazette},
    VOLUME = {57},
      YEAR = {1973},
    NUMBER = {400},
     PAGES = {87--94},
      ISSN = {0025-5572},
   MRCLASS = {50B30},
  MRNUMBER = {0461269},
       DOI = {10.2307/3615344},
       URL = {https://doi.org/10.2307/3615344},
}

@article {C1,
    AUTHOR = {Coxeter, H. S. M.},
     TITLE = {Frieze patterns},
   JOURNAL = {Acta Arith.},
  FJOURNAL = {Polska Akademia Nauk. Instytut Matematyczny. Acta Arithmetica},
    VOLUME = {18},
      YEAR = {1971},
     PAGES = {297--310},
      ISSN = {0065-1036},
   MRCLASS = {10.55 (01.00)},
  MRNUMBER = {0286771},
MRREVIEWER = {D. A. Klarner},
       DOI = {10.4064/aa-18-1-297-310},
       URL = {https://doi.org/10.4064/aa-18-1-297-310},
}

@article {Assem1,
    AUTHOR = {Assem, Ibrahim and Reutenauer, Christophe and Smith, David},
     TITLE = {Friezes},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {225},
      YEAR = {2010},
    NUMBER = {6},
     PAGES = {3134--3165},
      ISSN = {0001-8708},
   MRCLASS = {13F60 (05A15 05C50 05C75 17B22)},
  MRNUMBER = {2729004},
MRREVIEWER = {Kyungyong Lee},
       DOI = {10.1016/j.aim.2010.05.019},
       URL = {https://doi.org/10.1016/j.aim.2010.05.019},
}

@article {FST,
    AUTHOR = {Fomin, Sergey and Shapiro, Michael and Thurston, Dylan},
     TITLE = {Cluster algebras and triangulated surfaces. {I}. {C}luster
              complexes},
   JOURNAL = {Acta Math.},
  FJOURNAL = {Acta Mathematica},
    VOLUME = {201},
      YEAR = {2008},
    NUMBER = {1},
     PAGES = {83--146},
      ISSN = {0001-5962},
   MRCLASS = {57Q15 (13F60 32G15 52B70)},
  MRNUMBER = {2448067},
MRREVIEWER = {Christof Gei\ss },
       DOI = {10.1007/s11511-008-0030-7},
       URL = {https://doi.org/10.1007/s11511-008-0030-7},
}

@article {FZ,
    AUTHOR = {Fomin, Sergey and Zelevinsky, Andrei},
     TITLE = {Cluster algebras. {I}. {F}oundations},
   JOURNAL = {J. Amer. Math. Soc.},
  FJOURNAL = {Journal of the American Mathematical Society},
    VOLUME = {15},
      YEAR = {2002},
    NUMBER = {2},
     PAGES = {497--529},
      ISSN = {0894-0347},
   MRCLASS = {16S99 (14M99 17B99)},
  MRNUMBER = {1887642},
MRREVIEWER = {Eric N. Sommers},
       DOI = {10.1090/S0894-0347-01-00385-X},
       URL = {https://doi.org/10.1090/S0894-0347-01-00385-X},
}
@article {BMRRT,
    AUTHOR = {Buan, Aslak Bakke and Marsh, Robert and Reineke, Markus and
              Reiten, Idun and Todorov, Gordana},
     TITLE = {Tilting theory and cluster combinatorics},
   JOURNAL = {Adv. Math.},
  FJOURNAL = {Advances in Mathematics},
    VOLUME = {204},
      YEAR = {2006},
    NUMBER = {2},
     PAGES = {572--618},
      ISSN = {0001-8708},
   MRCLASS = {16G20 (16G70 16S99)},
  MRNUMBER = {2249625},
MRREVIEWER = {Lidia Angeleri H\"ugel},
       DOI = {10.1016/j.aim.2005.06.003},
       URL = {https://doi.org/10.1016/j.aim.2005.06.003},
}

@article {Am,
    AUTHOR = {Amiot, Claire},
     TITLE = {Cluster categories for algebras of global dimension 2 and
              quivers with potential},
   JOURNAL = {Ann. Inst. Fourier (Grenoble)},
  FJOURNAL = {Universit\'e de Grenoble. Annales de l'Institut Fourier},
    VOLUME = {59},
      YEAR = {2009},
    NUMBER = {6},
     PAGES = {2525--2590},
      ISSN = {0373-0956},
   MRCLASS = {16E35 (13F60 16E45 16G20)},
  MRNUMBER = {2640929},
MRREVIEWER = {Gregoire Dupont},
       URL = {http://aif.cedram.org/item?id=AIF_2009__59_6_2525_0},
}

@article {CCh,
    AUTHOR = {Caldero, Philippe and Chapoton, Fr\'ed\'eric},
     TITLE = {Cluster algebras as {H}all algebras of quiver representations},
   JOURNAL = {Comment. Math. Helv.},
  FJOURNAL = {Commentarii Mathematici Helvetici. A Journal of the Swiss
              Mathematical Society},
    VOLUME = {81},
      YEAR = {2006},
    NUMBER = {3},
     PAGES = {595--616},
      ISSN = {0010-2571},
   MRCLASS = {16G20 (18E30)},
  MRNUMBER = {2250855},
       DOI = {10.4171/CMH/65},
       URL = {https://doi.org/10.4171/CMH/65},
}

@article {LS,
    AUTHOR = {Lee, Kyungyong and Schiffler, Ralf},
     TITLE = {Positivity for cluster algebras},
   JOURNAL = {Ann. of Math. (2)},
  FJOURNAL = {Annals of Mathematics. Second Series},
    VOLUME = {182},
      YEAR = {2015},
    NUMBER = {1},
     PAGES = {73--125},
      ISSN = {0003-486X},
   MRCLASS = {13F60 (05E15)},
  MRNUMBER = {3374957},
MRREVIEWER = {Alfredo N\'ajera Ch\'avez},
       DOI = {10.4007/annals.2015.182.1.2},
       URL = {https://doi.org/10.4007/annals.2015.182.1.2},
}




@article {BMR,
    AUTHOR = {Buan, Aslak Bakke and Marsh, Robert J. and Reiten, Idun},
     TITLE = {Cluster-tilted algebras},
   JOURNAL = {Trans. Amer. Math. Soc.},
  FJOURNAL = {Transactions of the American Mathematical Society},
    VOLUME = {359},
      YEAR = {2007},
    NUMBER = {1},
     PAGES = {323--332},
      ISSN = {0002-9947},
   MRCLASS = {16G20},
  MRNUMBER = {2247893},
MRREVIEWER = {Lidia Angeleri H\"ugel},
       DOI = {10.1090/S0002-9947-06-03879-7},
       URL = {https://doi.org/10.1090/S0002-9947-06-03879-7},
}
		
@article {JKS,
    AUTHOR = {Jensen, Bernt Tore and King, Alastair D. and Su, Xiuping},
     TITLE = {A categorification of {G}rassmannian cluster algebras},
   JOURNAL = {Proc. Lond. Math. Soc. (3)},
  FJOURNAL = {Proceedings of the London Mathematical Society. Third Series},
    VOLUME = {113},
      YEAR = {2016},
    NUMBER = {2},
     PAGES = {185--212},
      ISSN = {0024-6115},
   MRCLASS = {13F60 (14M15 16G50 16S35)},
  MRNUMBER = {3534971},
MRREVIEWER = {Wen Chang},
       DOI = {10.1112/plms/pdw028},
       URL = {https://doi.org/10.1112/plms/pdw028},
}

@article {Ma,
    AUTHOR = {Magnani, Kodjo Essonana},
     TITLE = {Friezes of type {$\Bbb D$}},
   JOURNAL = {Rev. Un. Mat. Argentina},
  FJOURNAL = {Revista de la Uni\'on Matem\'atica Argentina},
    VOLUME = {58},
      YEAR = {2017},
    NUMBER = {2},
     PAGES = {227--243},
      ISSN = {0041-6932},
   MRCLASS = {13F60 (16G20)},
  MRNUMBER = {3733204},
MRREVIEWER = {Jiarui Fei},
}
	@article{FT18,
  title={Cluster algebras and triangulated surfaces part II: Lambda lengths},
  author={Fomin, Sergey and Thurston, Dylan},
  year={2018},
  publisher={American Mathematical Society}
}


@article {HJ,
    AUTHOR = {Holm, Thorsten and J\o rgensen, Peter},
     TITLE = {Generalised friezes and a modified {C}aldero-{C}hapoton map
              depending on a rigid object, {II}},
   JOURNAL = {Bull. Sci. Math.},
  FJOURNAL = {Bulletin des Sciences Math\'ematiques},
    VOLUME = {140},
      YEAR = {2016},
    NUMBER = {4},
     PAGES = {112--131},
      ISSN = {0007-4497},
   MRCLASS = {18D10 (05E10 13F60 16G70)},
  MRNUMBER = {3498312},
MRREVIEWER = {Ibrahim Saleh},
       DOI = {10.1016/j.bulsci.2015.05.001},
       URL = {https://doi.org/10.1016/j.bulsci.2015.05.001},
}


@article{MSW,
  title={Positivity for cluster algebras from surfaces},
  author={Musiker, Gregg and Schiffler, Ralf and Williams, Lauren},
  journal={Advances in Mathematics},
  volume={227},
  number={6},
  pages={2241--2308},
  year={2011},
  publisher={Elsevier}
}

@article {FP,
    AUTHOR = {Fontaine, Bruce and Plamondon, Pierre-Guy},
     TITLE = {Counting friezes in type {$D_n$}},
   JOURNAL = {J. Algebraic Combin.},
  FJOURNAL = {Journal of Algebraic Combinatorics. An International Journal},
    VOLUME = {44},
      YEAR = {2016},
    NUMBER = {2},
     PAGES = {433--445},
}

@article{P05,
  title={The combinatorics of frieze patterns and Markoff numbers},
  author={Propp, James},
  journal={arXiv preprint math/0511633},
  year={2005}
}

